Hierarchical Needs Based Self-Adaptive Framework For Cooperative Multi-Robot System

Research in multi-robot and swarm systems has seen significant interest in cooperation of agents in complex and dynamic environments. To effectively adapt to unknown environments and maximize the utility of the group, robots need to cooperate, share information, and make a suitable plan according to the specific scenario. Inspired by Maslow's hierarchy of human needs and systems theory, we introduce Robot's Need Hierarchy and propose a new solution called Self-Adaptive Swarm System (SASS). It combines multi-robot perception, communication, planning, and execution with the cooperative management of conflicts through a distributed Negotiation-Agreement Mechanism that prioritizes robot's needs. We also decompose the complex tasks into simple executable behaviors through several Atomic Operations, such as selection, formation, and routing. We evaluate SASS through simulating static and dynamic tasks and comparing them with the state-of-the-art collision-aware task assignment method integrated into our framework.

==> bib_original.tex <==
\begin{thebibliography}{99}

\bibitem{1} Serena Chan. ``Complex Adaptive Systems.'' MIT ESD.83 Research Seminar in Engineering Systems October 31, 2001/November 6, 2001.
\bibitem{2} Levin SA. ``Ecosystems and the biosphere as complex adaptive systems.'' Ecosystems, 1(5):431-6. 1998.
\bibitem{3} Beni G., Wang, J. ``Swarm Intelligence in Cellular Robotic Systems.'' In Proc. NATO Advanced Workshop on Robots and Biological Systems, Tuscany, Italy, June 26-30 (1989).
\bibitem{4} L. E. Parker, Daniela Rus, and Gaurav Sukhatme. ``{Multiple Mobile Robot Systems}.'' Chapter 53 of Springer Handbook of Robotics, Second Edition, B. Siciliano and O. Khatib, editors, 2016, pp. 1362--1363.
\bibitem{6} A.I. Mourikis, S.I. ``Roumeliotis: Optimal sensor scheduling for resource-constrained localization of mobile robot formations.'' IEEE Trans. Robotics {\bf 22}(5), 917-931 (2006).
\bibitem{7} S. Kloder, S. Hutchinson. ``Path planning for permutation-invariant multirobot formations.'' IEEE Trans. Robotics {\bf 22}(4), 650-665 (2006).
\bibitem{8} C.W. Reynolds. ``Flocks, herds and schools: A distributed behavioral model.'' ACM SIGGRAPH Comput. Gr. {\bf 21}, 25–34 (1987).
\bibitem{9} M.J. Mataric. ``Designing emergent behaviors: From local interactions to collective intelligence,.'' Proc. 2nd Int. Conf. Simul. Adapt. Behav. (1992) pp. 432-441.
\bibitem{10} T. Balch, R. Arkin. ``Behavior-based formation control for multi-robot teams.'' IEEE Trans. Robotics Autom. {\bf 14}(6), 926-939 (1998).
\bibitem{11} Y. Cao, W. Yu, W. Ren, G. Chen. ``An overview of recent progress in the study of distributed multi- agent coordination.'' IEEE Trans. Ind. Inf. {\bf 9}(1), 427-438 (2012).
\bibitem{12} R.M. Murray. ``Recent research in cooperative control of multi-vehicle systems.'' J. Dyn. Syst. Meas. Control {\bf 129}(5), 571-583 (2007).
\bibitem{13} Santoro N. ``Design and analysis of distributed algorithms.'' John Wiley \& Sons; 2006 Nov 3.
\bibitem{14} Erciyes K. ``Distributed graph algorithms for computer networks.'' Springer Science \& Business Media; 2013 May 16.
\bibitem{15} George Coulouris, Jean Dollimore, Tim Kindberg, Gordon Blair. ``{Distributed Systems Concepts and Design}.'' Fifth Edition, 2012
\bibitem{16} Gerhard Weiss, {Multiagent System}, Second Edition, 2013.
\bibitem{17} Jeff S. Shamma. ``{Cooperative Control of Distributed Multi-Agent Systems}.'' 2007.
\bibitem{18} John H. Holland, {Daedalus}, Vol. 121, No. 1, A New Era in Computation (Winter, 1992), pp. 17-30.
\bibitem{19} H. Wang, A. Kolling, N. Brooks, S. Owens, S. Abedin, P. Scerri, P.-j. Lee, S.-Y. Chien, M. Lewis, and K. Sycara. ``Scalable target detection for large robot teams.'' In Proc. of the 6th international conference on Human-robot interaction. ACM, 2011, pp. 363–370.
\bibitem{20} S. Swaminathan, M. Phillips, and M. Likhachev. ``Planning for multi- agent teams with leader switching.'' In 2015 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2015, pp. 5403–5410.
\bibitem{21} G. Wagner and H. Choset. ``Subdimensional expansion for multirobot path planning.'' Artificial Intelligence, vol. 219, pp. 1–24, 2015.
\bibitem{22} W. Luo, N. Chakraborty, and K. Sycara. ``Distributed dynamic priority assignment and motion planning for multiple mobile robots with kin- odynamic constraints.'' In 2016 American Control Conference (ACC). IEEE, 2016, pp. 148–154.
\bibitem{23} V. R. Desaraju and J. P. How. ``Decentralized path planning for multi- agent teams with complex constraints.'' Autonomous Robots, vol. 32, no. 4, pp. 385–403, 2012.
\bibitem{24} R. Olfati-Saber. ``Flocking for multi-agent dynamic systems: Algorithms and theory.'' IEEE Transactions on automatic control, vol. 51, no. 3, pp. 401–420, 2006.
\bibitem{25} G. Antonelli, F. Arrichiello, and S. Chiaverini. ``Flocking for multi- robot systems via the null-space-based behavioral control.'' Swarm Intelligence, vol. 4, no. 1, pp. 37–56, 2010.
\bibitem{26} M. M. Zavlanos, A. Jadbabaie, and G. J. Pappas. ``Flocking while preserving network connectivity.'' In 2007 46th IEEE Conference on Decision and Control. IEEE, 2007, pp. 2919–2924.
\bibitem{27} X. Yan, J. Chen, and D. Sun. ``Multilevel-based topology design and shape control of robot swarms.'' Automatica, vol. 48, no. 12, pp. 3122– 3127, 2012.
\bibitem{28} C. Belta and V. Kumar. ``Abstraction and control for groups of robots.'' IEEE Transactions on Robotics, vol. 20, no. 5, pp. 865–875, 2004.
\bibitem{29} N. Ayanian and V. Kumar.  ``Abstractions and controllers for groups of robots in environments with obstacles.'' In 2010 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2010, pp. 3537–3542.
\bibitem{30} H Hamann, H Wörn. ``A framework of space–time continuous models for algorithm design in swarm robotics.'' Swarm Intelligence, December 2008, 2(4), pp 209–-239.
\bibitem{31} Martinoli, A. ``Swarm intelligence in autonomous collective robotics: from tools to the analysis and synthesis of distributed control strategies.'' Ph.D. thesis, Ecole Polytechnique Féderale de Lausanne, 1999.
\bibitem{32} H. Hamann. ``Swarm Robotics: A Formal Approach.'' Springer, New York, 2018.
\bibitem{33} Winfield, A. F. T., Sav, J., Fernández-Gago, M.-C., Dixon, C., \& Fisher, M. `` On formal specification of emergent behaviours in swarm robotic systems.'' International Journal of Advanced Robotic Systems, 2(4), 2005. pp. 363-–370.
\bibitem{34} Soysal, O., Sahin, E. ``A macroscopic model for self-organized aggregation in swarm robotic systems.'' In E. Sahin, W. M. Spears, \& A. F. Winfield (Eds.), Lecture notes in computer science: Vol. 4433. pp. 27-–42. 2005. Berlin: Springer.
\bibitem{35} Gazi, V., Passino, K. M. ``Stability analysis of swarms.'' IEEE Transactions on Automatic Control, 48(4), 692–697. 2003.
\bibitem{36} Feddema, J. T., Lewis, C., \& Schoenwald, D. A. ``Decentralized control of cooperative robotic vehicles: theory and application.'' IEEE Transactions on Robotics and Automation, 18(5), 852–864. 2002.
\bibitem{37} Maslow A.H. ``A Theory of Human Motivation.'' Psychological Review, 50(4), 370-396. 1943.
\bibitem{38} Savage EL, Schruben LW. ``Eliminating event cancellation in discrete event simulation.'' In Proc. of the 27th Conference on Winter simulation 1995 (pp. 744-750). IEEE Computer Society.

\bibitem{39} Dahl J, Chetlur M, Wilsey PA. ``Event list management in distributed simulation.'' In European Conference on Parallel Processing 2001 Aug 28 (pp. 466-475). Springer, Berlin, Heidelberg.

\bibitem{40} Henderson TR, Lacage M, Riley GF, Dowell C, Kopena J. ``Network simulations with the ns-3 simulator.'' SIGCOMM demonstration. 2008 Aug 17;14(14):527.

\bibitem{41} Michael Otte, Michael Kuhlman, and Donald Sofge. ``Auctions for Multi-Robot Task Allocation in Communication Limited Environments.'' Autonomous Robots. pp 1-38, 29 January, 2019.
\bibitem{42} R. G. Smith and R. Davis. ``Frameworks for co-operation in distributed problem solving.'' IEEE Transaction on System, Man and Cybernetics, vol. 11, no. 1, 1981.
\bibitem{43} Samir Aknine, Suzanne Pinson, Melvin F. Shakun. ``An Extended Multi-Agent Negotiation Protocol.'', Autonomous Agents and Multi-Agent Systems, Jan 2004, 8(1).
\bibitem{44} Danny Weyns, Nelis Boucke, Tom Holvoet and Bart Demarsin. ``DynCNET: A Protocol for Dynamic Task Assignment in Multiagent Systems.''  First International Conference on Self-Adaptive and Self-Organizing Systems (SASO 2007).

\bibitem{45} Yang GZ, Bellingham J, Dupont PE, Fischer P, Floridi L, Full R, Jacobstein N, Kumar V, McNutt M, Merrifield R, Nelson BJ. ``The grand challenges of Science Robotics. Science Robotics.`` Science Robotics, 2018 Jan 31;3(14):eaar7650.

\bibitem{46} Colledanchise M, Ögren P. ``Behavior trees in robotics and AI: an introduction.'' CRC Press. 2018.
\bibitem{47} Colledanchise M, Parasuraman RN, Ogren P. ``Learning of behavior trees for autonomous agents.'' IEEE Transactions on Games. 2018 Mar 19.

\bibitem{48} Valencia R, Andrade-Cetto J. ``Active pose SLAM.'' In Mapping, Planning and Exploration with Pose SLAM 2018 (pp. 89--108). Springer, Cham.
\bibitem{49} Ahrenholz J.`` Comparison of CORE network emulation platforms.'' In 2010 Military Communications (Milcom) Conference 2010 Oct 31 (pp. 166--171). IEEE.

\end{thebibliography}

==> bibliography_ordered.tex <==
\begin{thebibliography}{99}



@incollection{valencia2018active,
  title={Active pose SLAM},
  author={Valencia, Rafael and Andrade-Cetto, Juan},
  booktitle={Mapping, Planning and Exploration with Pose SLAM},
  pages={89--108},
  year={2018},
  publisher={Springer}
}









\iffalse
\bibitem{6} A.I. Mourikis, S.I. ``Roumeliotis: Optimal sensor scheduling for resource-constrained localization of mobile robot formations.'' IEEE Trans. Robotics {\bf 22}(5), 917-931 (2006).
\bibitem{13} Santoro N. ``Design and analysis of distributed algorithms.'' John Wiley \& Sons; 2006 Nov 3.
\bibitem{14} Erciyes K. ``Distributed graph algorithms for computer networks.'' Springer Science \& Business Media; 2013 May 16.
\bibitem{15} George Coulouris, Jean Dollimore, Tim Kindberg, Gordon Blair. ``{Distributed Systems Concepts and Design}.'' Fifth Edition, 2012
\bibitem{16} Gerhard Weiss, {Multiagent System}, Second Edition, 2013.
\bibitem{17} Jeff S. Shamma. ``{Cooperative Control of Distributed Multi-Agent Systems}.'' 2007.
\bibitem{18} John H. Holland, {Daedalus}, Vol. 121, No. 1, A New Era in Computation (Winter, 1992), pp. 17-30.
\bibitem{19} H. Wang, A. Kolling, N. Brooks, S. Owens, S. Abedin, P. Scerri, P.-j. Lee, S.-Y. Chien, M. Lewis, and K. Sycara. ``Scalable target detection for large robot teams.'' In Proc. of the 6th international conference on Human-robot interaction. ACM, 2011, pp. 363–370.
\bibitem{20} S. Swaminathan, M. Phillips, and M. Likhachev. ``Planning for multi- agent teams with leader switching.'' In 2015 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2015, pp. 5403–5410.
\bibitem{25} G. Antonelli, F. Arrichiello, and S. Chiaverini. ``Flocking for multi- robot systems via the null-space-based behavioral control.'' Swarm Intelligence, vol. 4, no. 1, pp. 37–56, 2010.
\bibitem{26} M. M. Zavlanos, A. Jadbabaie, and G. J. Pappas. ``Flocking while preserving network connectivity.'' In 2007 46th IEEE Conference on Decision and Control. IEEE, 2007, pp. 2919–2924.
\bibitem{28} C. Belta and V. Kumar. ``Abstraction and control for groups of robots.'' IEEE Transactions on Robotics, vol. 20, no. 5, pp. 865–875, 2004.
\bibitem{38} Savage EL, Schruben LW. ``Eliminating event cancellation in discrete event simulation.'' In Proc. of the 27th Conference on Winter simulation 1995 (pp. 744-750). IEEE Computer Society.
\bibitem{39} Dahl J, Chetlur M, Wilsey PA. ``Event list management in distributed simulation.'' In European Conference on Parallel Processing 2001 Aug 28 (pp. 466-475). Springer, Berlin, Heidelberg.
\fi

\end{thebibliography}
